Lorentz group equivariant autoencoders

There has been significant work recently in developing machine learning (ML) models in high energy physics (HEP) for tasks such as classification, simulation, and anomaly detection. Often these models are adapted from those designed for datasets in computer vision or natural language processing, which lack inductive biases suited to HEP data, such as equivariance to its inherent symmetries. Such biases have been shown to make models more performant and interpretable, and reduce the amount of training data needed. To that end, we develop the Lorentz group autoencoder (LGAE), an autoencoder model equivariant with respect to the proper, orthochronous Lorentz group $\mathrm{SO}^+(3,1)$, with a latent space living in the representations of the group. We present our architecture and several experimental results on jets at the LHC and find it outperforms graph and convolutional neural network baseline models on several compression, reconstruction, and anomaly detection metrics. We also demonstrate the advantage of such an equivariant model in analyzing the latent space of the autoencoder, which can improve the explainability of potential anomalies discovered by such ML models.

==> sections/archive/GNNAE.tex <==
As a baseline model, we construct an autoencoder composed of fully-connected MPNNs adapted from \ccite{Raghav_GAN}, which has a high performance on this dataset. Detailed about the architecture can be found in \cref{app:hyperparams}.
% The update rule in the $(t+1)$-th MPNN layer is given by
% \begin{align}
%     m_i^{(t)} &= \sum_{j=1}^n f_e^{(t)}\left( 
%         x_i^{(t)} \oplus x_j^{(t)} \oplus d\left(x_i^{(t)}, x_j^{(t)}\right)
%     \right), \label{eq:gnnae-m} \\
%     x_i^{(t+1)} &= f_n^{(t)} \left(
%         x_i^{(t)} \oplus m_i^{(t)}
%     \right), \label{eq:gnnae-x}
% \end{align}
% where $x_i^{(t)}$ is the node embedding of node $i$ at $t$-th iteration, 
% $d$ is any distance function (Euclidean norm in our case), 
% $m_i^{(t)}$ is the message for updating node embedding in node $i$,
% $f_e^{(t+1)}$ and $f_n^{(t+1)}$ are any learnable mapping at the current MP layer.

We thereafter call it GNNAE (Graph Neural Network Autoencoder). The architecture for MP and the choice of hyperparameters are shown in \cref{app:hyperparams}.
However, the GNNAE models were not able to learn the substructure with 4-momenta input, so the GNNAEs were trained directly with $(p_\mathrm{T}^\mathrm{rel}, \eta^\mathrm{rel}, \phi^\mathrm{rel})$.

The best permutation invariant aggregation method for the GNNAE is jet-level aggregation, which takes the mean aggregation over the graph.
GNNAEs with jet-level aggregation are going to be compared directly with LGAEs with min-max aggregation because LGAEs resort to jet-level compression by taking the min and max aggregation over the graph, and in doing so, have permutation invariance.
GNNAEs with jet-level aggregation are trained with the Chamfer loss.

Another aggregation method is the particle-level aggregation~\cite{pgae}, which performs the mixing operation features in each node. We found that particle-level aggregation results in a better performance than jet-level aggregation. As a result, the GNNAE preserves the permutation symmetry by being permutation equivariant.
As the best-performing models of GNNAEs, GNNAEs with particle-level aggregation are going to be compared with mix aggregation so that we can compare the improvements after embedding the permutation symmetry and after embedding the Lorentz symmetry.
GNNAEs with particle-level aggregation are trained with the MSE loss.

==> sections/archive/computational-cost.tex <==
In terms of training time, we see from \cref{sec:training} that, in general, the LGAEs converge faster and train faster than the best-performing GNNAEs.

Another measure of computation cost is the number of learnable parameters for each model. We found that for our choice of MPNN layers, the number of learnable parameters $N$ of the LGAE models depends linearly on the multiplicity of latent 4-vectors, with $N$ given by
\begin{equation}
    N_\text{LGAE-Mix}(\tau_{(1/2, 1/2)}) = 62636 + 300 \tau_{(1/2, 1/2)} % \in O(\tau_{(1/2, 1/2)})
\end{equation}
for LGAE-Mix models, and
\begin{equation}
    N_\text{LGAE-Min-Max}(\tau_{(1/2, 1/2)}) = 62404 + 68 \tau_{(1/2, 1/2)} % \in O(\tau_{(1/2, 1/2)})
\end{equation}
for LGAE-Min-Max models.
Hence, the number of learnable parameters in the LGAE models grows linearly on the compression rate.
In our case, $N_\mathrm{particles} = 30$, so
\begin{equation}
    \label{eq:num-param-lgae}
    \begin{split}
        N_\text{LGAE-Mix}(\mathrm{CR}) &= 62561 + 4500 \mathrm{CR}, \\
        N_\text{LGAE-Min-Max}(\mathrm{CR}) &= 62387 + 510 \mathrm{CR},
    \end{split}
\end{equation}
for LGAE-Mix and LGAE-Min-Max respectively.
In the case of compression, the constant term dominates, so both aggregations result in $\mathcal{O}(65000)$ parameters.

For the GNNAEs, we found that the number of learnable parameters grows quadratically on the latent dimension size; given $N_\mathrm{particles}$ particles to reconstruct and the latent dimension $D=\dim(L)$, the number of learnable parameters
\begin{equation}
    \begin{split}
        N_\text{GNNAE-JL}(D) &= 6000 D^2 +  480 D + 27800 % \in O(D^2), \\
        N_\text{GNNAE-PL}(d) &= d^2 + 6 d + 27872 % \in O(d^2),
    \end{split}
\end{equation}
for GNNAE-JL and GNNAE-PL, respectively. Note that for convenience, we use $d = D / N_\mathrm{particles}$, that is the dimension per node, to parametrize the latent space of GNNAE-PL.
Hence, the number of learnable parameters in the GNNAE depends quadratically on the compression rate.
In the case of compression, $D \in [1, 90) \cap \mathbb{Z}^+$ and $d = \{1,2\}$, so the range of $N$ for each aggregation is given by
\begin{equation}
    \begin{split}
        N_\text{GNNAE-JL} &\in [31280, 2.383352 \times 10^7], \\
        N_\text{GNNAE-PL} &\in \{27879, 27888\}.
    \end{split}
\end{equation}
In our case, $N_\mathrm{particles} = 30$, so $D = 30 \mathrm{CR}$, and therefore
the numbers of learnable parameters are given by
\begin{equation}
    \label{eq:num-param-gnnae}
    \begin{split}
        N_\text{GNNAE-JL}(\mathrm{CR}) &= (2.43 \times 10^7) \mathrm{CR}^2 + 43200 \mathrm{CR} + 27800, \\
        N_\text{GNNAE-PL}(\mathrm{CR}) &= 9 \mathrm{CR}^2 + 18 \mathrm{CR} + 27872
    \end{split}
\end{equation}
for GNNAE-JL and GNNAE-PL, respectively.

From \cref{eq:num-param-lgae,eq:num-param-gnnae}, we see that an LGAE-Min-Max model requires fewer parameters than a GNNAE-JL model when the compression level satisfies $\mathrm{CR} > 3.7\%$, at which the latent dimension is $\dim(L) \geq 4$ and $\tau_{(1/2, 1/2)} \geq 1$. However, a latent dimension of $3$ is not practical for GNNAEs if we want an acceptable performance. At a practical compression level, the GNNAE-JL model will be much larger than the LGAE-Min-Max model. For instance, at about $50\%$, a GNNAE-JL model requires about $100$ times as many parameters as an LGAE-Min-Max model does.
Nevertheless, GNNAE-PL models are not always desirable because of the limited choice of compression levels.
In the case of compressing and reconstructing $(p_\mathrm{T}, \eta^\mathrm{rel}, \phi^\mathrm{rel})$, the only choices of GNNAE-PL are one with latent dimension $\dim(L) \in \{1 \times 30, 2 \times 30\}$.
By contrast, the latent 4-vector multiplicity, $\tau_{(1/2, 1/2)}$, in LGAE-Mix models can vary from $1$ to $14$, depending on the desired trade-off between reconstruction and compression.



==> sections/archive/hyperparams.tex <==
For both encoder and decoder, we choose $N_\mathrm{MP}^\mathrm{E} = N_\mathrm{MP}^\mathrm{D} = 4$ LMP layers.
The multiplicity per node in each LMP layer has been optimized to be
\begin{equation}
    \left\{ \parenthesis{\tau_{(m, n)}^{(t)}}^\mathrm{E} \right\}_{t=1}^{4} = (3,3,4,4)
\end{equation}
for the encoder and
\begin{equation}
    \left\{ \parenthesis{\tau_{(m, n)}^{(t)}}^\mathrm{D} \right\}_{t=1}^{4} = (4,4,3,3)
\end{equation}
for the decoder.
After each CG decomposition, we truncate irreps of higher dimensions than $(1/2, 1/2)$ for tractable computations.
As a result, $(m,n) \in \{(0,0), (1/2, 1/2)\}$.
Empirically, we did not find such a truncation to affect the performance of the model.

The differentiable mapping $f(d_{ij})$ in \cref{eq:msg} is chosen to be the Lorentzian bell function as in Ref.~\cite{LGN}.
For all models, the latent space contains only $\tau_{(0,0)} = 1$ complex Lorentz scalar, as increasing this does not improve the performance in either reconstruction or anomaly detection.
This is probably because the original dataset does not have intrinsic scalars to learn from other than the invariant mass, which derives from a 4-vector.

For models with the min-max aggregation, we chose the multiplicity of complexified Lorentz vectors to range from $1$ ($16.7\%$ compression) and $7$ ($96.7\%$ compression).
For models with the mixing operation in the layer of the encoder, we chose the multiplicity of complexified Lorentz vectors to range from $1$ ($8.3\%$ compression) and $13$ ($88.3\%$ compression).

==> sections/archive/loss.tex <==
% As the network is permutation invariant with respect to the input particles, we expect to require a permutation invariant loss function as well. 
For models with permutation invariant aggregations,
we experiment with three permutation-invariant loss functions, the Chamfer distance~\cite{10.5555/1622943.1622971,Fan_2017_CVPR,Zhang2020FSPool} between the input and output set of particles,
% \begin{equation}
%     \mathcal{L}(J_1, J_2) = \sum_{\mathbf{p}_1 \in J_1} \min_{\mathbf{p}_2 \in J_2} |\mathbf{p}_1 - \mathbf{p}_2|^2 + \sum_{\mathbf{p}_2 \in J_2} \min_{\mathbf{p}_1 \in J_1} |\mathbf{p}_1 - \mathbf{p}_2|^2,
% \end{equation}
% where $J_1$ and $J_2$ are two jets, 
the Hungarian loss calculated via the Hungarian method~\cite{hungarian} using the Scipy library~\cite{scipy},
and a differentiable energy mover's distance (EMD)~\cite{emd},
calculated using the JetNet library~\cite{jetnetlibrary}. The EMD finds the minimum ``work'' needed, in terms of transverse momentum flows, to rearrange the particle constituents from one jet to the other.
We also test the permutation-symmetry-breaking mean-squared error (MSE) between the final list of particles as a baseline, expecting the former two permutation-invariant losses to perform better.

We used the Chamfer loss function~\cite{10.5555/1622943.1622971,Fan_2017_CVPR,Zhang2020FSPool} for LGAEs with min, max, and mean aggregation and GNNAEs with mean aggregation and the MSE loss for LGAEs and GNNAEs with mix aggregation. We also tested the Hungarian loss~\cite{hungarian,scipy} and differentiable energy mover's distance (EMD)~\cite{emd} calculated using the JetNet library~\cite{jetnetlibrary}, but we found the former to be the most performant.

==> sections/archive/tables-anomaly.tex <==
\begin{table*}[htpb]
    \centering
    \caption{
        Anomaly detection metrics by a selection of LGAE models with min-max and mix aggregations and with different multiplicities of latent 4-vectors ($\tau_{(1/2, 1/2)})$
    }
    \label{tab:lgae-ad}
    \begin{tabular}{c|c|c|c|c|c} \toprule
        \multirow{2}{*}{Aggregation} & \multirow{2}{*}{$\tau_{(1/2,1/2)}$} & \multirow{2}{*}{AUC} &
        \multicolumn{3}{|c}{$\varepsilon_s$ at given $1 - \varepsilon_b$}
        \\ \cline{4-6}
                                     &                                     &                      & $\varepsilon_s (10^{-1})$ & $\varepsilon_s (10^{-2})$ & $\varepsilon_s (10^{-3})$         \\ \hline
        \multirow{3}{*}{min-max}
        % & $1$ ($16.67\%$) & $0.7129$ & $0.5173$ & $0.1082$ & $0.8865 \times 10^{-3}$ \\
                                     & $2$ ($30.00\%$)                     & $0.7253$             & $0.5706$                  & $0.1130$                  & $\mathbf{1.1686} \times 10^{-3}$  \\
        % & $3$ ($43.33\%$) & $0.7428$ & $0.5822$ & $0.0036$ & $1.0074 \times 10^{-3}$ \\
                                     & $4$ ($56.67\%$)                     & $0.7627$             & $0.5832$                  & $\mathbf{0.1305}$         & $0.6850 \times 10^{-3}$           \\
        % & $5$ ($70.00\%$) & $0.7281$ & $0.5661$ & $0.0036$ & $0.3224 \times 10^{-3}$ \\
        % & $6$ ($83.33\%$) & $0.6933$ & $0.0702$ & $0.0061$ & $0.7656 \times 10^{-3}$ \\
                                     & $7$ ($96.67\%$)                     & $\mathbf{0.7673}$    & $\mathbf{0.5932}$         & $0.0820$                  & $0.9268 \times 10^{-3}$           \\
        \hline
        \multirow{3}{*}{mix}
        % & $1$ ($8.33\%$) & $0.7987$ & $0.6065$ & $0.1640$ & $24.4600 \times 10^{-3}$ \\
                                     & $2$ ($15.00\%$)                     & $\mathbf{0.8023}$    & $0.6178$                  & $\mathbf{0.1662}$         & $\mathbf{25.0242} \times 10^{-3}$ \\
        % & $3$ ($21.67\%$) & $0.8022$ & $0.6229$ & $0.1610$ & $23.6138 \times 10^{-3}$ \\
                                     & $4$ ($28.33\%$)                     & $\mathbf{0.8023}$    & $0.6257$                  & $0.1592$                  & $22.9288 \times 10^{-3}$          \\
        % & $5$ ($35.00\%$) & $0.8011$ & $0.6285$ & $0.1561$ & $22.7676 \times 10^{-3}$ \\
        % & $6$ ($41.67\%$) & $0.7984$ & $0.6278$ & $0.1543$ & $22.0422 \times 10^{-3}$ \\
                                     & $7$ ($48.33\%$)                     & $0.7967$             & $\mathbf{0.6290}$         & $0.1562$                  & $22.4855 \times 10^{-3}$          \\
        % & $8$ ($55.00\%$) & $0.7945$ & $0.6271$ & $0.1553$ & $22.3243 \times 10^{-3}$ \\
        % & $9$ ($61.67\%$) & $0.7924$ & $0.6253$ & $0.1551$ & $21.9616 \times 10^{-3}$ \\
        % & $10$ ($68.33\%$) & $0.7908$ & $0.6229$ & $0.1539$ & $21.9213 \times 10^{-3}$ \\
        % & $11$ ($75.00\%$) & $0.7896$ & $0.6195$ & $0.1538$ & $21.5587 \times 10^{-3}$ \\
        % & $12$ ($81.67\%$) & $0.7885$ & $0.6162$ & $0.1528$ & $21.0348 \times 10^{-3}$ \\
        % & $13$ ($88.33\%$) & $0.7877$ & $0.6136$ & $0.1507$ & $21.1557 \times 10^{-3}$ \\
        \bottomrule
    \end{tabular}
\end{table*}

\begin{table*}[htpb]
    \centering
    \caption{Anomaly detection metrics by GNNAE models with mean aggregation, particle-level aggregation, and event-level aggregation and with different choices of latent space ($L$) dimension}
    \label{tab:gnnae-ad}
    \begin{tabular}{c|c|c|c|c|c} \toprule
        \multirow{2}{*}{Aggregation} & \multirow{2}{*}{$\dim (L)$} & \multirow{2}{*}{AUC} &
        \multicolumn{3}{|c}{$\varepsilon_s$ at given $1 - \varepsilon_b$}
        \\ \cline{4-6}
                                     &                             &                      & $\varepsilon_s (10^{-1})$ & $\varepsilon_s (10^{-2})$ & $\varepsilon_s (10^{-3})$       \\ \hline
        \multirow{3}{*}{mean}
                                     & $10$ ($11.11\%$)            & $0.5891$             & $0.1576$                  & $0.0161$                  & $\mathbf{1.426} \times 10^{-3}$ \\
        % & $20$ ($22.22\%$) & $0.6738$ & $0.2139$ & $0.0214$ & $1.138 \times 10^{-3}$ \\
        % & $30$ ($33.33\%$) & $0.6638$ & $0.2114$ & $0.0197$ & $0.897 \times 10^{-3}$ \\
                                     & $40$ ($44.44\%$)            & $0.6636$             & $\mathbf{0.2293}$         & $\mathbf{0.0262}$         & $1.257 \times 10^{-3}$          \\
        % & $45$ ($50.00\%$) & $0.6496$ & $0.2171$ & $0.0239$ & $1.028 \times 10^{-3}$ \\
        % & $50$ ($55.56\%$) & $0.5560$ & $0.1824$ & $0.0189$ & $0.956 \times 10^{-3}$ \\
        % & $60$ ($66.67\%$) & $0.6887$ & $0.2250$ & $0.0227$ & $1.077 \times 10^{-3}$ \\
        % & $70$ ($77.78\%$) & $0.5912$ & $0.1998$ & $0.0212$ & $1.206 \times 10^{-3}$ \\
                                     & $80$ ($88.89\%$)            & $\mathbf{0.7006}$    & $0.2240$                  & $0.0239$                  & $1.001 \times 10^{-3}$          \\
        \hline
        \multirow{2}{*}{event-level compression}
        % & $10$ ($11.11\%$) & $0.7506$ & $0.2424$ & $0.0337$ & $3.850 \times 10^{-3}$ \\
        % & $20$ ($22.22\%$) & $0.7709$ & $0.2733$ & $0.0390$ & $3.112 \times 10^{-3}$ \\
        % & $30$ ($33.33\%$) & $0.7209$ & $0.2470$ & $0.0257$ & $2.011 \times 10^{-3}$ \\
        % & $40$ ($44.44\%$) & $0.7302$ & $0.2346$ & $0.0280$ & $3.413 \times 10^{-3}$ \\
                                     & $45$ ($50.00\%$)            & $\mathbf{0.8100}$    & $0.3524$                  & $0.0442$                  & $4.328 \times 10^{-3}$          \\
        % & $50$ ($55.56\%$) & $0.8049$ & $0.3943$ & $0.0473$ & $4.288 \times 10^{-3}$ \\
                                     & $60$ ($66.67\%$)            & $0.7935$             & $\mathbf{0.4294}$         & $\mathbf{0.0892}$         & $\mathbf{6.339} \times 10^{-3}$ \\
        % & $70$ ($77.78\%$) & $0.7372$ & $0.2617$ & $0.0234$ & $1.743 \times 10^{-3}$ \\
        % & $90$ ($100.00\%$) & $0.7361$ & $0.2427$ & $0.0171$ & $0.913 \times 10^{-3}$ \\
        \hline
        \multirow{2}{*}{particle-level compression}
        % & $1$ ($33.33\%$) & $0.7700$ & $0.3444$ & $0.0546$ & $6.511 \times 10^{-3}$ \\
                                     & $2$ ($66.67\%$)             & $\mathbf{0.8195}$    & $\mathbf{0.4435}$         & $0.0564$                  & $4.164 \times 10^{-3}$          \\
                                     & $3$ ($100.00\%$)            & $0.8095$             & $0.4306$                  & $\mathbf{0.0762}$         & $\mathbf{4.436} \times 10^{-3}$ \\
        \bottomrule
    \end{tabular}
\end{table*}

==> sections/archive/tables-recons.tex <==
\begin{table*}[htpb]
    \centering
    \caption{Median, IQR, IDR, and MAD of relative errors in particle feature reconstructions
        % $(p_\mathrm{T}^\mathrm{rel}, \eta^\mathrm{rel}, \phi^\mathrm{rel})$ 
        by LGAE models with min-max and mean aggregations and different latent 4-vector multiplicities ($\tau_{(1/2, 1/2}))$}
    \label{tab:lgae-rel-err}
    \begin{tabular}{c|c|c|c|c|c}  \toprule
        Aggregation & $\tau_{(1/2,1/2)}$ & Median             & IQR               & IDR               & MAD               \\ \hline
        \multirow{4}{*}{mix}
                    & $1$ ($8.33\%$)     & $-0.9937$          & $0.3073$          & $1.1156$          & $0.2282$          \\
        % & $2$ ($15\%$) & $-0.9133$ & $0.8151$ & $2.3117$ & $0.5999$ \\
        % & $3$ ($21.7\%$) & $-0.8284$ & $1.0682$ & $2.5809$ & $0.7771$ \\
        % & $4$ ($28.3\%$) & $-0.7430$ & $1.1802$ & $2.6592$ & $0.9027$ \\
        % & $5$ ($35\%$) & $-0.6469$ & $1.1518$ & $2.6003$ & $0.9290$ \\
        % & $6$ ($41.7\%$) & $-0.5186$ & $1.0790$ & $2.4694$ & $0.7692$ \\
        % & $7$ ($48.3\%$) & $-0.3383$ & $0.9979$ & $2.3223$ & $0.5915$ \\
                    & $8$ ($55\%$)       & $-0.1044$          & $0.9017$          & $2.1050$          & $0.5624$          \\
        % & $9$ ($61.7\%$) & $-0.0268$ & $0.7908$ & $1.7971$ & $0.3152$ \\
                    & $10$ ($68.3\%$)    & $-0.0070$          & $0.6487$          & $1.5860$          & $0.1130$          \\
        % & $11$ ($75\%$) & $-0.0046$ & $0.4483$ & $1.3469$ & $0.0507$ \\
        % & $12$ ($81.7\%$) & $-0.0020$ & $0.1333$ & $1.0439$ & $0.0218$ \\
                    & $13$ ($88.3\%$)    & $\mathbf{-0.0010}$ & $\mathbf{0.0334}$ & $\mathbf{0.7337}$ & $\mathbf{0.0162}$ \\
        \hline
        \multirow{3}{*}{min-max}
                    & $1$ ($16.7\%$)     & $-0.9187$          & $0.6578$          & $3.6695$          & $0.4223$          \\
        % & $2$ ($30\%$) & $-0.8598$ & $0.7858$ & $5.0929$ & $0.4391$ \\
        % & $3$ ($43.3\%$) & $-0.8144$ & $0.7667$ & $2.1915$ & $0.5064$ \\
                    & $4$ ($56.7\%$)     & $-0.8273$          & $\mathbf{0.5908}$ & $\mathbf{1.5687}$ & $\mathbf{0.3783}$ \\
        % & $5$ ($70\%$) & $-0.6906$ & $0.9988$ & $4.9665$ & $0.6737$ \\
        % & $6$ ($83.3\%$) & $-0.7892$ & $0.7963$ & $2.1898$ & $0.5136$ \\
                    & $7$ ($96.7\%$)     & $\mathbf{-0.6611}$ & $1.0231$          & $3.1747$          & $0.7145$          \\
        \bottomrule
    \end{tabular}
\end{table*}

\begin{table*}[htpb]
    \centering
    \caption{Statistical information of relative errors of particle feature reconstructions $(p_\mathrm{T}^\mathrm{rel}, \eta^\mathrm{rel}, \phi^\mathrm{rel})$ by GNNAE models with mean aggregation, particle-level compression, and event-level compression and different choices of latent space ($L$) dimension}
    \label{tab:gnnae-rel-err}
    \begin{tabular}{c|c|c|c|c|c} \toprule
        Aggregation & $\mathrm{dim}(L)$        & Median             & IQR               & IDR               & MAD               \\
        \hline
        \multirow{2}{*}{mean}
        % & $10$ ($11.11\%$) & $-0.3751$ & $66.2510$ & $311.5367$ & $45.5576$ \\
        % & $20$ ($22.22\%$) & $-0.6437$ & $2.7995$ & $33.1554$ & $2.0685$ \\
        % & $30$ ($33.3\%$) & $-0.3154$ & $100.0672$ & $406.3601$ & $74.1706$ \\
        % & $40$ ($44.44\%$) & $8.8350$ & $95.8544$ & $434.4220$ & $71.0152$ \\
                    & $45$ ($50\%$)            & $-0.9206$          & $\mathbf{0.9358}$ & $\mathbf{9.1956}$ & $\mathbf{0.6824}$ \\
        % & $50$ ($55.56\%$) & $5.1683$ & $194.8777$ & $749.3679$ & $144.4135$ \\
        % & $60$ ($66.7\%$) & $-0.7489$ & $85.6550$ & $381.3820$ & $63.4941$ \\
        % & $70$ ($77.78\%$) & $16.4635$ & $90.4129$ & $347.8333$ & $53.3769$ \\
        % & $80$ ($88.89\%$) & $-0.8951$ & $1.5038$ & $31.1750$ & $1.0992$ \\
                    & $90$ ($100\%$)           & $\mathbf{-0.5746}$ & $3.0710$          & $46.0842$         & $2.2745$          \\
        \hline
        \multirow{2}{*}{event-level compression}
        % & $10$ ($11.11\%$) & $-0.9486$ & $0.8226$ & $3.2387$ & $0.5905$ \\
        % & $20$ ($22.22\%$) & $-0.4852$ & $1.0965$ & $3.1037$ & $0.8160$ \\
        % & $30$ ($33.33\%$) & $1.0000$ & $0.2847$ & $2.4263$ & $0.2110$ \\
        % & $40$ ($44.44\%$) & $-0.4696$ & $1.0980$ & $2.5751$ & $0.8162$ \\
        % & $45$ ($50.00\%$) & $-0.0635$ & $0.6498$ & $1.8415$ & $0.2866$ \\
        % & $50$ ($55.56\%$) & $-0.0509$ & $0.5917$ & $1.6848$ & $0.2450$ \\
        % & $60$ ($66.67\%$) & $-0.0073$ & $0.0995$ & $0.7589$ & $0.0648$ \\
                    & $70$ ($77.78\%$)         & $-0.0037$          & $\mathbf{0.0473}$ & $\mathbf{0.3281}$ & $\mathbf{0.0330}$ \\
                    & $80$ ($88.89\%$)         & $\mathbf{-0.0035}$ & $0.0721$          & $0.3506$          & $0.0517$          \\
        % & $90$ ($100.00\%$) & $-0.0048$ & $0.0676$ & $0.3376$ & $0.0477$ \\
        \hline
        \multirow{2}{*}{particle-level compression}
        % & $1 \times 30$ ($33.3\%$) & $-0.0616$ & $0.5993$ & $3.0333$ & $0.4156$ \\
                    & $2 \times 30$ ($66.7\%$) & $\mathbf{-0.0164}$ & $\mathbf{0.1347}$ & $2.1180$          & $\mathbf{0.0815}$ \\
                    & $3 \times 30$ ($100\%$)  & $-0.0235$          & $0.3612$          & $\mathbf{1.9607}$ & $0.1784$          \\
        \bottomrule
    \end{tabular}
\end{table*}

==> sections/archive/training.tex <==
We used the Chamfer loss function~\cite{10.5555/1622943.1622971,Fan_2017_CVPR,Zhang2020FSPool} for LGAEs with min, max, and mean aggregation and GNNAEs with mean aggregation and the MSE loss for LGAEs with mix aggregation and GNNAEs with particle-level aggregation.
We also tested the Hungarian loss~\cite{hungarian,scipy} and differentiable energy mover's distance (EMD)~\cite{emd} calculated using the \jetnet library~\cite{jetnetlibrary}, but we found the former to be the most performant.

The LGAE models were optimized by the Adam optimizer \cite{ADAM}
implemented in PyTorch \cite{pytorch}
with a learning rate $\gamma = 10^{-3}$, coefficients $(\beta_1, \beta_2) = (0.9, 0.999)$, and weight decay $\lambda = 0$.
The LGAE models with the mix aggregations and MSE loss as the objective function
and LGAE models with the min-max aggregations and Chamfer loss as the objective function
were each trained on single NVIDIA RTX 2080 Ti GPUs each for 2000 epochs with early stopping.
Most models converge within the first $400$ epochs but were trained to improve marginally until the set patience ($200$ stale epochs) hit. The total training time is typically 35 hours and at most 100 hours. with a typical total epoch of 400 and a maximum total epoch of 1200.

The baseline GNNAE models were trained on the same dataset with the same optimizer and the same setting.
The GNNAE models with global aggregation were trained with MSE loss, and those with mean aggregation were trained with Chamfer loss.
Different from LGAE models, GNNAE models with particle-level aggregation take at least $700$ epochs to converge, taking about $50$ hours in total; and GNNAE models with even-level aggregation take at least $2000$ epochs to converge, taking about $120$ hours in total.
